Hard X-ray emission from extragalactic IRAS 12um sources: constraints on the unified AGN model and the synthesis of the X-ray background

We analyze the $2-10$~keV X-ray emission of complete samples of AGN and galaxies selected at 12$\mu$m and recently compiled by Rush, Malkan \& Spinoglio (1993). As a necessary complement we also study the IR emissivity of the largest sample of hard X--ray selected AGN (Grossan 1992). Our purposes are to probe the unified scheme of active nuclei and to evaluate the local X--ray volume emissivity of low luminosity and `hidden' AGN. We confirm that X-ray emission is basically restricted to AGN, Seyfert 1's being much more powerful emitters than Seyfert 2's. We find no signal of X-ray emission for the remaining galaxies selected at $12\mu$m, not even for those having a flat far-infrared spectrum, which would be prime candidates to host hidden AGN. Our result on the local volume emissivity of the Seyfert 1's is fully consistent with those derived from studies of the hard X--ray luminosity function. However the 95$\%$ upper limits to the local emissivity we derive for the Seyfert 2 class and for the most likely `hidden' AGN candidates, severely constrain (and in some cases exclude) models of the X--ray background based on the unified Seyfert scheme. We also find that less than $\sim20$\% of Seyfert 1-like AGN and less than $\sim 50$\% of Seyfert 2-like AGN can be `hidden' in the non-Seyfert galaxy samples assuming that the X-ray to 12$\mu$m flux ratios measured in the 12$\mu$m selected samples can be considered typical for these classes of objects. In this case, the number ratio of Seyfert 2 to Seyfert 1 galaxies ranges from 1 to 2.

==> iras12-tab1.tex <==
%   !!!!!!!!!!  This is table 1. Plain TEX  !!!!!!!!!!!!!
\magnification=\magstep1
\baselineskip=0.8truecm
\vsize=17truecm
\hsize=24truecm
\nopagenumbers

\noindent{\bf Table 1.} Results of the search of $f_X/f_{12\mu}$ for different
 subsamples. Error ranges and upper limits quoted correspond to 95 per cent
confidence. Estimates of 2-10 keV volume emissivities for the various 
samples.

\vskip 2truecm

\settabs 6\columns

\hrule

\medskip

\+Sample&No. Sources&X-ray Band&Significance&$f_X/f_{12\mu}$ & $j_X(z=0) $ \cr

\smallskip

\+      &           &  &(\%)    &     &  $h_{50}\, {\rm erg}\, {\rm s}^{-1}\, {\rm
Mpc}^{-3}$ \cr

\medskip

\hrule

\medskip

\+Seyfert 1&\hfill 54\hfill&Total& $>99.9999$&$(1.4_{-0.4}^{+1.1})\times 10^{-6}$
&$(2.1_{-0.6}^{+1.7})\times 10^{38}$\cr
\+Seyfert 1 $L_{12\mu}<10^{30}$&\hfill 33\hfill& Total& $> 99.999$&
$(1.2_{-0.4}^{+1.8})\times 10^{-6}$ & \cr
\+Seyfert 1 $L_{12\mu}>10^{30}$&\hfill 21\hfill& Total& $\sim 95$&$ (1.6_{-1.2}^{+1.2})\times
10^{-6}$ & \cr
\+Seyfert 1&\hfill 54\hfill &Hard&$>99$& $(1.4_{-0.8}^{+1.2})\times 10^{-6}$ & \cr
\+Seyfert 2&\hfill 59\hfill &Total& $\sim 95$ &$(2.0_{-1.5}^{+4.5})\times 10^{-7}$ 
&$(0.26_{-0.20}^{+0.58})\times 10^{38}$\cr
\+Seyfert 2&\hfill 59\hfill&Hard&$\sim 85$& $(3_{-3}^{+4})\times 10^{-7}$ & \cr
\+Hot Dust Galaxies&\hfill 152\hfill &Total&$<70$&$<1.0\times 10^{-7}$
&$<0.9 \times 10^{38}$\cr
\+Galaxies&\hfill 721\hfill&Total&$<70$&$<0.8 \times 10^{-7}$
&$<3.4 \times 10^{38}$\cr
\+All&\hfill 835\hfill &Total&$>95$&$(0.8_{-0.6}^{+0.6}) \times 10^{-7}$
&$(3.6_{-2.7}^{+2.8})\times 10^{38}$\cr

\medskip

\hrule

\bye




==> iras12-tab2.tex <==
\magnification=\magstep1
\vsize=17truecm
\hsize=24truecm
\baselineskip=0.8truecm
\nopagenumbers

\noindent{\bf Table 2.} Cross-Correlation Function of different galaxy
catalogues with the A2 sky map and inferred volume emissivities. Quoted errors
and upper limits refer to the 95\% level (obtained by bootstrapping
techniques).

\vskip 2truecm

\settabs 6\columns

\hrule

\medskip

\+Sample&Source density&$R_{\star}$&$R_{clus}$&CCF&$j_X(z=0)$\cr

\+      & (sources/beam)& (Mpc) & (Mpc) &     & $h_{50}\, {\rm erg}\, {\rm s}^{-1}\, {\rm
Mpc}^{-3}$\cr


\medskip

\hrule

\medskip

\+Seyfert 1&$1.04\times 10^{-2}$&$108_{-21}^{+28}$&$0.6_{-0.1}^{+0.1}$
&$(1.14_{-0.3}^{+1.1})\times 10^{-1}$&$(1.7_{-0.7}^{+2.4})\times
10^{38}$\cr
\+Seyfert 2&$1.15\times 10^{-2}$&$94_{-21}^{+32}$&
$0.7_{-0.1}^{+0.1}$&$(3.1_{-2.2}^{+4.8})\times 10^{-2}$&
$(0.57_{-0.44}^{+1.37})\times 10^{38}$\cr
\+Hot Dust Galaxies&$2.9\times 10^{-2}$&$68_{-8}^{+9}$&
$2.4_{-0.2}^{+0.2}$&$(1.7_{-15}^{+11})\times 10^{-3}$&
$<0.92\times 10^{38}$\cr
\+Galaxies&$1.4\times 10^{-1}$&$57_{-5}^{+5}$&
$12_{-0.5}^{+0.5}$&$(0.3_{-15}^{+11})\times 10^{-3}$&
$<3.73\times 10^{38}$\cr
\+All&$1.6\times 10^{-1}$&$61_{-1}^{+5}$&$13.5_{-0.5}^{+0.5}$
&$(9.0_{-9.6}^{+13})\times 10^{-3}$&
$<7.8\times 10^{38}$\cr

\medskip

\hrule

\bye




==> iras12-tab3.tex <==
\magnification=\magstep1
\baselineskip=0.8truecm
\nopagenumbers

\noindent {\bf Table 3.} Non linear fits to the $L_X$ vs $L_{12}$ relation
for Seyfert 1 galaxies selected at $12\mu$m as defined by eq. (2). For the
listed values of the slope $b$, the normalisation $a$ is fitted by means
of the IDA.  



\vskip 2truecm

\settabs 2 \columns

\hrule

\medskip

\+ $b$ & $a$ \cr

\medskip

\hrule

\medskip

\+  1.20 &  $-12.0\pm 0.25$\cr
\+  1.25 &  $-13.6\pm 0.25$\cr
\+  1.30 &  $-15.1\pm 0.25$\cr
\+  1.40 &  $-18.2\pm 0.25$\cr


\medskip

\hrule

\bye


